Faster and Sample Near-Optimal Algorithms for Proper Learning Mixtures of Gaussians

We provide an algorithm for properly learning mixtures of two single-dimensional Gaussians without any separability assumptions. Given $\tilde{O}(1/\varepsilon^2)$ samples from an unknown mixture, our algorithm outputs a mixture that is $\varepsilon$-close in total variation distance, in time $\tilde{O}(1/\varepsilon^5)$. Our sample complexity is optimal up to logarithmic factors, and significantly improves upon both Kalai et al., whose algorithm has a prohibitive dependence on $1/\varepsilon$, and Feldman et al., whose algorithm requires bounds on the mixture parameters and depends pseudo-polynomially in these parameters. One of our main contributions is an improved and generalized algorithm for selecting a good candidate distribution from among competing hypotheses. Namely, given a collection of $N$ hypotheses containing at least one candidate that is $\varepsilon$-close to an unknown distribution, our algorithm outputs a candidate which is $O(\varepsilon)$-close to the distribution. The algorithm requires ${O}(\log{N}/\varepsilon^2)$ samples from the unknown distribution and ${O}(N \log N/\varepsilon^2)$ time, which improves previous such results (such as the Scheff\'e estimator) from a quadratic dependence of the running time on $N$ to quasilinear. Given the wide use of such results for the purpose of hypothesis selection, our improved algorithm implies immediate improvements to any such use.

==> closestpoint.tex <==
\section{Robust Estimation of Scale from a Mixture of Gaussians}
In this section, we examine the following statistic:

Given some point $x \in \mathbb{R}$ and $n$ IID random variables $X_1, \dots, X_n$, what is the minimum distance between $x$ and any $X_i$?

We give an interval in which this statistic is likely to fall (Proposition \ref{closept}), and examine its robustness when sampling from distributions which are statistically close to the distribution under consideration (Proposition \ref{closeptrob}).
We then apply these results to mixtures of Gaussians (Proposition \ref{closeptgmm} and Lemma \ref{closeptgmmrob}).

\begin{proposition}
  \label{closept}
  Suppose we have $n$ IID random variables $X_1, \dots, X_n \sim X$, some $x \in \mathbb{R}$, and $y = F_X(x)$.
  Let $I_L$ be the interval $[F_X^{-1}(y - \frac{c_2}{n}), F_X^{-1}(y - \frac{c_1}{n})]$ and
      $I_R$ be the interval $[F_X^{-1}(y + \frac{c_1}{n}), F_X^{-1}(y + \frac{c_2}{n})]$ for some constants $0 < c_1 < c_2 \leq n$, and $I = I_L \cup I_R$.
      Let $j = \arg\min_i |X_i - x|$.
      Then $\Pr[X_j \in I] \geq \frac{9}{10}$ for all $n > 0$.
\end{proposition}
\begin{proof}
  We show that $\Pr[X_j \not \in I] \leq \frac{1}{10}$ by showing that the following two bad events are unlikely:
  \begin{enumerate}
    \item We have a sample which is too close to $x$
    \item All our samples are too far from $x$
  \end{enumerate}
  Showing these events occur with low probability and combining with the union bound gives the desired result.

  Let $Y$ be the number of samples at distance $< \frac{c_1}{n}$ in distance in the CDF, i.e., $Y = |\{i\mid|F_X^{-1}(X_i) - y| < \frac{c_1}{n}\}|$.
  By linearity of expectation, $E[Y] = 2c_1$.
  By Markov's inequality, $\Pr(Y > 0) < 2c_1$.
  This allows us to upper bound the probability that one of our samples is too close to $x$.

  Let $Z$ be the number of samples at distance $< \frac{c_2}{n}$ in distance in the CDF, i.e., $Z = |\{i\mid|F_X^{-1}(X_i) - y| < \frac{c_2}{n}\}|$, and let $Z_i$ be an indicator random variable which indicates this property for $X_i$.
  We use the second moment principle,
  $$\Pr(Z > 0) \geq \frac{E[Z]^2}{E[Z^2]}$$
  By linearity of expectation, $E[Z]^2 = 4c_2^2$.
  \begin{align*}
    E[Z^2] &= \sum_i E[Z_i^2] + \sum_i \sum_{j \neq i} E[Z_iZ_j] \\
           &= 2c_2 + n(n-1)\left(\frac{4c_2^2}{n^2}\right) \\
           &\geq 2c_2 + 4c_2^2
  \end{align*}
  And thus, $\Pr(Z = 0) \leq \frac{1}{2c_2+1}$.
  This allows us to upper bound the probability that all of our samples are too far from $x$.

  Setting $c_1 = \frac{1}{40}$ and $c_2 = \frac{19}{2}$ gives probability $< \frac{1}{20}$ for each of the bad events, resulting in a probability $< \frac{1}{10}$ of either bad event by the union bound, and thus the desired result.
\end{proof}

The next proposition says that if we instead draw samples from a distribution which is close in total variation distance, the same property approximately holds with respect to the original distribution.
\begin{proposition}
  \label{closeptrob}
  Suppose we have $n$ IID random variables $\hat X_1, \dots, \hat X_n \sim \hat X$ where $d_{TV}(f_X,f_{\hat X}) \leq \d$, some $x \in \mathbb{R}$, and $y = F_X(x)$.
  Let $I_L$ be the interval $[F_X^{-1}(y - \frac{c_2}{n} - 2\d), F_X^{-1}(y - \frac{c_1}{n} + 2\d)]$ and
      $I_R$ be the interval $[F_X^{-1}(y + \frac{c_1}{n} - 2\d), F_X^{-1}(y + \frac{c_2}{n} + 2\d)]$ for some constants $0 < c_1 < c_2 \leq n$, and $I = I_L \cup I_R$.
      Let $j = \arg\min_i |X_i - a|$.
      Then $\Pr[X_j \in I] \geq \frac{9}{10}$ for all $n > 0 $.
\end{proposition}
\begin{proof}
  First, apply Proposition \ref{closept} to $\hat X$ to find that $X_j$ will lie in one of the two intervals
  $\hat I_L = [F_{\hat X}^{-1}(y - \frac{c_2}{n}), F_{\hat X}^{-1}(y - \frac{c_1}{n})]$ or
  $\hat I_R = [F_{\hat X}^{-1}(y + \frac{c_1}{n}), F_{\hat X}^{-1}(y + \frac{c_2}{n})]$ with probability $\geq \frac{9}{10}$.
  However, these intervals are in terms of $F_{\hat X}$ instead of $F_{X}$ - the remainder of the proof consists of constructing $I_L \supseteq \hat I_L$ and $I_R \supseteq \hat I_R$, where the two new intervals are described in terms of $F_X$.
  We will show that the left endpoint of $I_R$ is to the left of the left endpoint of $\hat I_R$, the other three endpoints can be analyzed similarly.

  Let $L = F_X^{-1}(y + \frac{c_1}{n})$ and $\hat L = F_{\hat X}^{-1}(y + \frac{c_1}{n})$.
  $\hat L$ will be the left endpoint of the interval $\hat I_R$.
  By the definition of $\hat L$, we know its location with respect to $F_{\hat X}$.
  We wish to bound its position with respect to $F_{X}$, showing that it is not ``too close'' to $x$:
  in particular, we want to show $F_X(\hat L) - F_X(x) > \frac{c_1}{n} - 2\d$.

  Since $d_{TV}(f_X,f_{\hat X}) \leq \d$, we can deduce the following:
  \begin{align*}
    \d &\geq \frac12\int_{-\infty}^{\infty}\! |f_{\hat X}(z) - f_X(z)|\, \mathrm{d}z \\
       &\geq \frac12\int_{x}^{\hat L}\! |f_{\hat X}(z) - f_{X}(z)|\, \mathrm{d}z \\
       &\geq \frac12\int_{x}^{\hat L}\! f_{\hat X}(z) - f_{X}(z)\, \mathrm{d}z \\
       &= \frac12\frac{c_1}{n}- \frac12\int_{x}^{\hat L}\! f_{X}(z)\, \mathrm{d}z \\
  \end{align*}
  where the equality is by the definition of $\hat L$.
  By rearranging, we see 
  $$\int_{x}^{\hat L}\! f_{X}(z)\, \mathrm{d}z \geq \frac{c_1}{n} - 2\d$$
  This implies that $\hat L > F_{X}^{-1}(y + \frac{c_1}{n} - 2\d)$, giving the desired result.
\end{proof}

We examine this statistic for some mixture of $k$ Gaussians with PDF $f$ around the point corresponding to the mean of the component with the minimum value of $\frac{\s_i}{w_i}$.
Initially, we assume that we know this location exactly and that we are taking samples according to $f$ exactly.

\begin{proposition}
  \label{closeptgmm}
  Consider a mixture of $k$ Gaussians with PDF $f$, components $\mathcal{N}(\m_1,\s_1^2), \dots, \mathcal{N}(\m_k, \s_k^2)$ and weights $w_1, \dots, w_k$.
  Let $j = \arg\min_i \frac{\s_i}{w_i}$.
  If we take $n$ samples $X_1,\dots,X_n$ from the mixture (where $n > \frac{3\sqrt{\p}c_2}{2w_j}$), then
  $\min_i |X_i - \m_j| \in [\frac{\sqrt{2\p}c_1\s_j}{kw_jn},\frac{3\sqrt{2\p}c_2\s_j}{2w_jn}]$ with probability $\geq \frac{9}{10}$, where $c_1$ and $c_2$ are as defined in Proposition \ref{closept}.
\end{proposition}
\begin{proof}
  We examine the CDF of the mixture around $\m_i$.
  Using Proposition 1 (and symmetry of a Gaussian about its mean), it is sufficient to show that
  $[\m_i + \frac{\sqrt{2\p}c_1\s_i}{kw_in},\m_i + \frac{3\sqrt{2\p}c_2\s_i}{2w_in}] \supseteq
[F^{-1}(F(\m_i) + \frac{c_1}{n}), F^{-1}(F(\m_i) + \frac{c_2}{n})]$, where $F$ is the CDF of the mixture.
  We show that each endpoint of the latter interval bounds the corresponding endpoint of the former interval.

  First, we show $\frac{c_1}{n} \geq F(\m_i +\frac{\sqrt{2\p}c_1\s_i}{kw_in}) -  F(\m_i)$.
  Let $I = [\m_i, \m_i + \frac{\sqrt{2\p}c_1\s_i}{kw_in}]$, $f$ be the PDF of the mixture, and $f_i$ be the PDF of component $i$ of the mixture.
  The right-hand side of the inequality we wish to prove is equal to 
  \begin{align*}
    \int_{I}\! f(x)\, \mathrm{d}x &= \int_{I}\! \sum_{j=1}^k w_jf_j(x)\, \mathrm{d}x \\
                                  &\leq \int_{I}\! \sum_{j=1}^k w_j\frac{1}{\s_j\sqrt{2\p}}\, \mathrm{d}x \\
                                  &\leq \int_{I}\! \frac{kw_i}{\s_i\sqrt{2\p}}\, \mathrm{d}x \\
                                  &= \frac{c_1}{n}
  \end{align*}
  where the first inequality is since the maximum of the PDF of a Gaussian is $\frac{1}{\s\sqrt{2\p}}$, and the second is since $\frac{\s_j}{w_j} \leq \frac{\s_i}{w_i}$ for all $j$.
  

  Next, we show $\frac{c_2}{n} \leq F(\m_i + \frac{3\sqrt{2\p}c_2\s_i}{2w_in}) -  F(\m_i)$.
  We note that the right-hand side is the probability mass contained in the interval - a lower bound for this quantity is the probability mass contributed by the particular Gaussian we are examining, which is $\frac{w_i}{2}\erf{\left(\frac{3\sqrt{\p}c_2}{2w_in}\right)}$.
  Taking the Taylor expansion of the error function gives
  $$\erf(x) = \frac{2}{\sqrt{\p}}\left(x -\frac{x^3}{3} + O(x^5)\right) \geq \frac{2}{\sqrt{\p}}\left(\frac{2}{3}x\right)$$
  if $x < 1$.
  Applying this here, we can lower bound the contributed probability mass by $\frac{w_i}{2}\frac{2}{\sqrt{\p}}\frac{2}{3}\frac{3\sqrt{\p}c_2}{2w_in} = \frac{c_2}{n}$, as desired.
\end{proof}

Finally, we deal with uncertainties in parameters and apply the robustness properties of Proposition \ref{closeptrob} in the following lemma:
\begin{lemma}
  \label{closeptgmmrob}
  Let $c_1$ and $c_2$ be constants as defined in Proposition \ref{closept}, and $c_3 = \frac{c_1}{9\sqrt{2}c_2}$.
  Consider a mixture of $k$ Gaussians $f$, with components $\mathcal{N}(\m_1,\s_1^2), \dots, \mathcal{N}(\m_k, \s_k^2)$ and weights $w_1, \dots, w_k$, and let $j = \arg\min_i \frac{\s_i}{w_i}$.
  Suppose we have estimates for the weights and means for all $i \in [1,k]$:
  \begin{itemize}
    \item $\hat w_i$, such that $\frac12 \hat w_i \leq w_i \leq 2\hat w_i$
    \item $\hat \mu_i$, such that $|\hat \mu_i - \mu_i| \leq \frac{c_3}{2k}\s_j$
  \end{itemize}
  Now suppose we draw $n = \frac{9\sqrt{\p}c_2}{2\hat w_j}$ samples $X_1, \dots, X_n$ from a distribution $\hat f$, 
  where $\dtv(f,\hat f) \leq \d = \frac{c_1}{4n} = \frac{c_1}{18\sqrt{\p}c_2}\hat w_j$.
  Then $\min_i |X_i - \hat \m_j| \in [\frac{c_3}{2k}\s_j, (\sqrt{2} + \frac{c_3}{2k})\s_j]$ with probability $\geq \frac{9}{10}$.
\end{lemma}
\begin{proof}
  We analyze the effect of each uncertainty:
  \begin{itemize}
    \item First, we consider the effect of sampling from $\hat f$, which is $\d$-close to $f$.
          By using Proposition \ref{closeptrob}, we know that the nearest sample to $\m_j$ 
          will be at CDF distance between $\frac{c_1}{n} - 2\d \geq \frac{c_1}{2n}$ 
          and $\frac{c_2}{n} + 2\d \leq \frac{3c_2}{2n}$.
          We can then repeat the proof of Proposition \ref{closeptgmm} 
          with $c_1$ replaced by $\frac{c_1}{2}$ and $c_2$ replaced by $\frac{3c_2}{2}$.
          This gives us that 
          $\min_i |X_i - \m_j| \in 
          [\frac{\sqrt{\p}c_1}{\sqrt{2}kw_jn}\s_j, \frac{9\sqrt{\p}c_2}{2\sqrt{2}w_jn}\s_j]$
          (where $n \geq \frac{9\sqrt{\p}c_2}{4w_j}$)
          with probability $\geq \frac{9}{10}$.
    \item Next, substituting in the bounds $\frac12\hat w_j \leq w_j \leq 2\hat w_j$, we get
          $\min_i |X_i - \m_j| \in 
          [\frac{\sqrt{\p}c_1}{2\sqrt{2}k\hat w_jn}\s_j, \frac{9\sqrt{\p}c_2}{\sqrt{2}\hat w_jn}\s_j]$
          (where $n \geq \frac{9\sqrt{\p}c_2}{2\hat w_j}$)
          with probability $\geq \frac{9}{10}$.
    \item We use $n = \frac{9\sqrt{\p}c_2}{2\hat w_j}$ samples to obtain:
          $\min_i |X_i - \m_j| \in 
          [\frac{c_3}{k}\s_j, \sqrt{2}\s_j]$
          with probability $\geq \frac{9}{10}$.
    \item Finally, applying $| \hat \m_j - \m_j| \leq \frac{c_3}{2k}\s_j$ gives the lemma statement.
  \end{itemize}
  
\end{proof}

